Vision Language Models are In-Context Value Learners

Predicting temporal progress from visual trajectories is important for intelligent robots that can learn, adapt, and improve. However, learning such progress estimator, or temporal value function, across different tasks and domains requires both a large amount of diverse data and methods which can scale and generalize. To address these challenges, we present Generative Value Learning (\GVL), a universal value function estimator that leverages the world knowledge embedded in vision-language models (VLMs) to predict task progress. Naively asking a VLM to predict values for a video sequence performs poorly due to the strong temporal correlation between successive frames. Instead, GVL poses value estimation as a temporal ordering problem over shuffled video frames; this seemingly more challenging task encourages VLMs to more fully exploit their underlying semantic and temporal grounding capabilities to differentiate frames based on their perceived task progress, consequently producing significantly better value predictions. Without any robot or task specific training, GVL can in-context zero-shot and few-shot predict effective values for more than 300 distinct real-world tasks across diverse robot platforms, including challenging bimanual manipulation tasks. Furthermore, we demonstrate that GVL permits flexible multi-modal in-context learning via examples from heterogeneous tasks and embodiments, such as human videos. The generality of GVL enables various downstream applications pertinent to visuomotor policy learning, including dataset filtering, success detection, and advantage-weighted regression -- all without any model training or finetuning.

==> oxe_rankings.tex <==
## Gemini
Task	Score
utokyo_pr2_opening_fridge_converted_externally_to_rlds	0.8095
utokyo_xarm_bimanual_converted_externally_to_rlds	0.7955
utokyo_xarm_pick_and_place_converted_externally_to_rlds	0.788
fractal20220817_data	0.7385
maniskill_dataset_converted_externally_to_rlds	0.726
berkeley_autolab_ur5	0.7185
nyu_door_opening_surprising_effectiveness	0.6685
utokyo_pr2_tabletop_manipulation_converted_externally_to_rlds	0.5875
utaustin_mutex	0.581
iamlab_cmu_pickup_insert_converted_externally_to_rlds	0.5585
fmb	0.5555
ucsd_kitchen_dataset_converted_externally_to_rlds	0.5295
dobbe	0.5295
toto	0.527
bridge	0.5145
austin_sirius_dataset_converted_externally_to_rlds	0.51
asu_table_top_converted_externally_to_rlds	0.5055
berkeley_rpt_converted_externally_to_rlds	0.4835
berkeley_cable_routing	0.447
usc_cloth_sim_converted_externally_to_rlds	0.441
jaco_play	0.4205
bc_z	0.4065
viola	0.4035
berkeley_mvp_converted_externally_to_rlds	0.39
roboturk	0.3545
austin_buds_dataset_converted_externally_to_rlds	0.3415
stanford_hydra_dataset_converted_externally_to_rlds	0.3325
tokyo_u_lsmo_converted_externally_to_rlds	0.314
berkeley_fanuc_manipulation	0.2685
cmu_stretch	0.2625
ucsd_pick_and_place_dataset_converted_externally_to_rlds	0.241
kuka	0.1915
dlr_sara_pour_converted_externally_to_rlds	0.16
taco_play	0.0945
dlr_edan_shared_control_converted_externally_to_rlds	0.0855
droid	-0.006
stanford_robocook_converted_externally_to_rlds	-0.069
imperialcollege_sawyer_wrist_cam	-0.1225
kaist_nonprehensile_converted_externally_to_rlds	-0.131
austin_sailor_dataset_converted_externally_to_rlds	-0.1715
cmu_play_fusion	-0.3445
stanford_kuka_multimodal_dataset_converted_externally_to_rlds	-0.377
stanford_mask_vit_converted_externally_to_rlds	-0.4505
nyu_franka_play_dataset_converted_externally_to_rlds	-0.4555
uiuc_d3field	-0.7025
cmu_franka_exploration_dataset_converted_externally_to_rlds	-0.7395
columbia_cairlab_pusht_real	-0.7625
robo_net	-0.8485
dlr_sara_grid_clamp_converted_externally_to_rlds	-1

## GPT
Task	Score
nyu_door_opening_surprising_effectiveness	0.883
utokyo_pr2_opening_fridge_converted_externally_to_rlds	0.864
berkeley_mvp_converted_externally_to_rlds	0.8285
utaustin_mutex	0.813
fractal20220817_data	0.803
utokyo_xarm_pick_and_place_converted_externally_to_rlds	0.7665
berkeley_autolab_ur5	0.755
utokyo_xarm_bimanual_converted_externally_to_rlds	0.749
utokyo_pr2_tabletop_manipulation_converted_externally_to_rlds	0.734
austin_sirius_dataset_converted_externally_to_rlds	0.7235
toto	0.713
dlr_edan_shared_control_converted_externally_to_rlds	0.6595
bridge	0.6445
berkeley_fanuc_manipulation	0.6295
berkeley_rpt_converted_externally_to_rlds	0.6235
ucsd_kitchen_dataset_converted_externally_to_rlds	0.603
roboturk	0.57
jaco_play	0.5615
iamlab_cmu_pickup_insert_converted_externally_to_rlds	0.557
uiuc_d3field	0.5395
usc_cloth_sim_converted_externally_to_rlds	0.5355
asu_table_top_converted_externally_to_rlds	0.5025
maniskill_dataset_converted_externally_to_rlds	0.499
kaist_nonprehensile_converted_externally_to_rlds	0.492
viola	0.4605
austin_buds_dataset_converted_externally_to_rlds	0.454
cmu_play_fusion	0.4235
tokyo_u_lsmo_converted_externally_to_rlds	0.3875
austin_sailor_dataset_converted_externally_to_rlds	0.3015
ucsd_pick_and_place_dataset_converted_externally_to_rlds	0.2675
berkeley_cable_routing	0.255
dlr_sara_pour_converted_externally_to_rlds	0.252
imperialcollege_sawyer_wrist_cam	0.239
robo_net	0.237
stanford_hydra_dataset_converted_externally_to_rlds	0.205
cmu_stretch	0.1895
bc_z	0.176
nyu_franka_play_dataset_converted_externally_to_rlds	0.1735
stanford_robocook_converted_externally_to_rlds	0.16
kuka	0.132
stanford_mask_vit_converted_externally_to_rlds	-0.173
stanford_kuka_multimodal_dataset_converted_externally_to_rlds	-0.1785
columbia_cairlab_pusht_real	-0.1815
cmu_franka_exploration_dataset_converted_externally_to_rlds	-0.2075
taco_play	-0.2705
eth_agent_affordances	-0.279
dlr_sara_grid_clamp_converted_externally_to_rlds	-1

